Learning User Embeddings from Temporal Social Media Data: A Survey

User-generated data on social media contain rich information about who we are, what we like and how we make decisions. In this paper, we survey representative work on learning a concise latent user representation (a.k.a. user embedding) that can capture the main characteristics of a social media user. The learned user embeddings can later be used to support different downstream user analysis tasks such as personality modeling, suicidal risk assessment and purchase decision prediction. The temporal nature of user-generated data on social media has largely been overlooked in much of the existing user embedding literature. In this survey, we focus on research that bridges the gap by incorporating temporal/sequential information in user representation learning. We categorize relevant papers along several key dimensions, identify limitations in the current work and suggest future research directions.

==> evaluation_method.tex <==
\section{Evaluation Method}
\fatema{This section is a good candidate for removal since this doesn't say anything to evaluate temporal embedding}
To assess the quality of the user embeddings 
There are a number of approaches to asses the quality of user embeddings; they broadly fall under to major categories: \textit{intrinsic} and \textit{extrinsic}. We discuss them in details below:

\paragraph{Intrinsic}
While measuring the performance of a user embedding on the downstream task can a good way to evaluate it effectiveness, there are cases when the downstream task might not be immediately obvious (e.g. learning a generalized embedding with a self-supervised objective). Hence, the \textit{intrinsic} evaluation metrics are designed to evaluate the quality and coherence of the vector space, independent from the downstream tasks. 
The primary objective here is to derive a measure of the semantic representations to assess the quality of the learnt user embedding.
The commonly used intrinsic measure for user representation learn is \textit{perplexity}, a lower perplexity score if indicative of a better generalization.
Among the paper we surveyed, ~\cite{sang2015probabilistic,liang2018dynamic} reported model performance using this metric. 
Computing the similarity between user embeddings is another popular intrinsic method; Both ~\cite{liang2018dynamic,beladev2020tdgraphembed} used cosine similarity in their evaluation where semantically similar have higher cosine similarity.
Other methods that compute similarity between users in the embedding space are Persons and Spearmans Correlation Coefficients, and the Jaccard Index~\cite{yin2015dynamic}.

% Rankisng Coefficient~\hl{need to correct it}.

\paragraph{Extrinsic}
As stated previously, measure the performance on the downstream task (if available) is the most direct way to assess the quality of the learn user embeddings, which we refer to as \textit{extrinsic} evaluation. 
Such evaluations are necessary to understand the effectiveness of different embedding techniques in real-world applications. 
Some of the most common downstream tasks used for extrinsic evaluation include personalized temporal recommendation~\cite{sang2015probabilistic,yin2014temporal,yin2015dynamic,fani2020user}, information diffusion prediction~\cite{gao2017novel,zhuo2019diffusiongan}, anomaly detection~\cite{yu2018netwalk,costa2017modeling}, fake account detection~\cite{noorshams2020ties}, node (user) classification~\cite{liu2020dynamic}, link (friendship) prediction~\cite{liu2020dynamic,xiong2019dyngraphgan} and photo popularity prediction~\cite{wu2016unfolding,wu2017sequential}.
If a user embedding consistently performs well in one or more of these downstream task compared to competing methods, the efficacy of the pertaining method can be well justified.  
